Fractional Payment Transactions: Executing Payment Transactions in Parallel with Less than f+1 Validations

We consider the problem of supporting payment transactions in an asynchronous system in which up to $f$ validators are subject to Byzantine failures under the control of an adaptive adversary. It was shown that, in the case of a single owner, this problem can be solved without consensus by using byzantine quorum systems (requiring a quorum of $2f+1$ validations per transaction). Nonetheless, the process of validating transactions remains sequential. For example, if one has a balance of ten coins and intends to make separate payments of two coins each to two distinct recipients, both transactions must undergo processing by a common correct validator. On the other hand, these two transactions are non-conflicting as they do not lead to double spending, allowing in principle for parallel validation. In this paper, we show that it is possible to validate payment transactions in parallel with less than $f$ validations per transaction in an asynchronous system, provided that each transaction spends only a small fraction of a balance. Our solution relies on a novel class of probabilistic quorum systems that we introduce in this paper, termed \textit{$(k_1,k_2)$-quorum systems}. In the absence of an adaptive adversary, \textit{$(k_1,k_2)$-quorum systems} can be used to enable concurrent and asynchronous validation of up to $k_1$ transactions while preventing validation of more than $k_2$ transactions. Employing a $(k_1, k_2)$-quorum system, we introduce protocols enabling a payer to validate multiple \textit{fractional spending} transactions in parallel with less than $f+1$ validations per transaction. Subsequently, the payer reclaims any remaining funds through a fully validated transaction, referred to as a \textit{settlement} transaction.

==> off-chain-partial-spending.tex <==

\section{Partial spending from partially validated funds}\label{sec:off-chain}
If a buyer pays a seller with a partial spending transaction, how can the seller turn around and spend some of the received amount without first settling the fund? It turns out, maybe not surprisingly, that in our asynchronous system model with an adaptive adversary, this does not seem to be achievable without some restrictions. One issue is the inability of the seller to prove to a potential buyer that it has a properly validated level-1 payment because that would require divulging the identities of the validators, which is problematic as we described. Also, it is not clear that a zero-knowledge proof of validity is possible. A seller who is the recipient of level-1 payment has only the validation from the buyer (the signatures of the hashes) that it can share as part of a level-2 payment. This would at least prevent a seller who has not received a level-1 payment from attempting to make a level-2 payment, but this is a weak guarantee because both the buyer and the seller can be corrupt.

We outline the main idea for supporting level-$i$ payments, but do not present any protocols. The idea for supporting level-$i$ payments, $i > 1$, is the following. We start with a buyer who has an fully certified fund. The buyer can make up to $k'_2$ level-1 partial spending transactions. If we want to spend from the resulting $k'_2$ funds (level-2 payments), we can have $k'_2$ partial spending transactions from each one of them, resulting in ${k'_2}^2$ level-2 partial spending transactions. So, in general, our approach will allow a total of ${k'_2}^i$ level-$i$ spending transactions, $i \geq 1$. 

Of course all of this should be done so that double spending is not possible.  For level-1 payments, the total spending can be as high as $k'_2 * F.\fbl/k'_2 = F.\fbl$, and potentially there might be no funds left for level-2 payments! One way to deal with this is to reduce the partial spending fraction from $1/k'_2$ to $1/2k'_2$.   This way, the total of level-1 payments is $k'_2 * F.\fbl/2k'_2 = F.\fbl/2$. The total for level-2 payments is ${k'_2}^2 * F.\fbl/4{k'_2}^2 = F.\fbl/4$. So the total spending at all levels is $F.\fbl/2 + F.\fbl/4 + F.\fbl/8 + \ldots \leq F.\fbl$. So, essentially, multi-level spending from partially certified funds can achieved by decreasing the amount that can be spent from a given balance. Also, it would require that the fund {\em level} be part of the fund description, which could be maintained as a chain of spending transactions starting from level-1 up to the level of the fund. 

One limitation of this approach is that it does not guarantee for every recipient of a level-1 payment the ability to make $k'_2$ level-2 payments. Instead, the guarantee is on the total number of level-2 payments. With this solution, a corrupt buyer, can issue many level-1 payments that are not properly validated to sellers under the control of the adversary. These sellers can then make level-2 payments that {\em consume} the total quota of level-2 payments. So, if the buyer is corrupt, a seller can be denied the opportunity to make level-2 payments, but the buyer's corruption will be detected. The situation can get worse as we go up the levels. Nonetheless, the fact that level-2 and higher payments can be made at all is surprising.

 

==> problem-definition.tex <==
\section{Problem Definition}\label{sec:definition}
Before presenting the requirements, we introduce some notation. For a given fund $F$, we denote by $\funds_F$ the set of funds resulting from payment transactions of the form $(F,\pkb,\pks, \text{PAY})$ and we denote by $\funds^H_F$  the set of 
such funds for which the seller $\pks$ is honest. 
We denote by $\settled_F$ the set of fully certified funds resulting from transactions of the form 
$(F_{pay},\text{SETTLE})$, where $F_{pay} \in \funds_F$; i.e. the set of settlement transactions of funds resulting from spending money from $F$. 

The following holds with high probability (we use {\em with high probability}, abbreviated \whp, to denote a probability of the form $1-\negl$, where $\negl$ is a negligible function in the relevant parameters): 

\begin{enumerate}
    \item (\textbf{progress}) All partially validated funds with honest owners can be settled successfully: Let $F'$ be a partially validated fund resulting from transaction $(F,\pkb,\pks, \mbox{PAY})$ where $F$ is a fully validated fund and $\pks$ is honest. If $\pks$ executes transaction  $(F',\text{SETTLE})$, the transaction will terminate resulting a fully validated fund. 
    
     \item (\textbf{safety}) If $F''$ is a fully validated fund resulting from executing $(F',\mbox{SETTLE})$ for partially validated fund $F'$, then $F''.\fbl = F'.\fbl$.  

     \item (\textbf{safety}) There can be at most $k'_2$ partial spending transactions of the form $(F,\pkb,\pks, \mbox{PAY})$, from a given fund $F$, for a total spending not exceeding $F.\fbl$.  
    
    \item (\textbf{safety}) Settlement amounts for payments from $F$ are subtracted from settlement for $F$:  If executing transaction $(F,\mbox{SETTLE})$ results in a fully validated fund $F_R$:
   $  F_R.\fbl \leq  F.\fbl - \sum_{F' \in \settled_F} F'.\fbl
   $ 
    
 \item (\textbf{safety}) Payments to honest sellers are subtracted from the settlement amount: 
    If executing transaction $(F,\mbox{SETTLE})$ results in a fully validated fund $F_R$: $F_R.\fbl \leq  F.\fbl - \sum_{F' \in \funds^H_F} F'.\fbl$
   
 \item (\textbf{safety}) If the owners of a fund $F$ are honest, the settlement amount is no less than the the initial balance of $F$ minus payments made from $F$:  
    If executing transaction $(F,\mbox{SETTLE})$ results in a fully validated fund $F_R$ and $F.\owners$ are honest:
     $  F_R.\fbl \geq F.\fbl - \sum_{F' \in \funds_F} F'.\fbl
    $
 
    
    \item (\textbf{progress}) Non-interference: If a total of $k \leq k_1$ payment transactions are initiated from fully validated fund $F$ and no additional payment or settlement transactions are initiated by $F.\owners$, then,  every one of the $k$ transactions whose seller (payee) is honest will be validated.  

\item (\textbf{progress}) 
Successful settlement for fully certified funds: If only one settlement transaction $(F,\mbox{SETTLE})$ is executed by one of the honest owners of a fully validated fund $F$ and no  $(F,\mbox{SETTLE})$ transaction is executed by any of the other owners, the settlement transaction for $F$ will terminate. 
\end{enumerate}

Note that, for the non-interference requirement, the guarantee of termination for each transaction holds even if the messages for the remaining transactions are arbitrarily delayed by slow sellers for example. In other words, executing one transaction does not interfere with the completion of other transactions if the total number of transactions does not exceed the threshold $k_1$.  Finally, note that termination of the execution of 
settlement transaction assumes that only one such transaction is
executed by one of the honest owners of the fund. 
